Spanning Training Progress: Temporal Dual-Depth Scoring (TDDS) for Enhanced Dataset Pruning

Dataset pruning aims to construct a coreset capable of achieving performance comparable to the original, full dataset. Most existing dataset pruning methods rely on snapshot-based criteria to identify representative samples, often resulting in poor generalization across various pruning and cross-architecture scenarios. Recent studies have addressed this issue by expanding the scope of training dynamics considered, including factors such as forgetting event and probability change, typically using an averaging approach. However, these works struggle to integrate a broader range of training dynamics without overlooking well-generalized samples, which may not be sufficiently highlighted in an averaging manner. In this study, we propose a novel dataset pruning method termed as Temporal Dual-Depth Scoring (TDDS), to tackle this problem. TDDS utilizes a dual-depth strategy to achieve a balance between incorporating extensive training dynamics and identifying representative samples for dataset pruning. In the first depth, we estimate the series of each sample's individual contributions spanning the training progress, ensuring comprehensive integration of training dynamics. In the second depth, we focus on the variability of the sample-wise contributions identified in the first depth to highlight well-generalized samples. Extensive experiments conducted on CIFAR and ImageNet datasets verify the superiority of TDDS over previous SOTA methods. Specifically on CIFAR-100, our method achieves 54.51% accuracy with only 10% training data, surpassing random selection by 7.83% and other comparison methods by at least 12.69%.

==> 4_Method.tex <==
\section{Methodology}
\label{sec:Methodology}
\begin{figure*}[h]
    \centering
    \includegraphics[width=0.85\linewidth]{figs/framework.pdf}
    \caption{The pipeline of our proposed TDDS. First, we record individual predicted probabilities of samples $f_{t_i}^{x_n} = f_{\bm{\theta}_{t_i}}(\bm{x}_n)$ during training. Then, we approximate the projected gradient, i.e. the component of gradient $\bm{g}_{t_i}^{x_n} = \bm{g}_{t_i}(\bm{x}_n)$ on accumulated gradient $\bm{G}_{t_i}$ direction, with KL-based loss difference between two adjacent epochs. Next, the projected gradients are used to estimate individual contributions of samples. Finally, the important samples are identified with larger projected gradient variances over time.}
    \label{fig:framework}
\end{figure*}
As discussed earlier, despite that exploring long-range dynamics provides a more comprehensive sample evaluation, the averaging operation hinders the construction of a coreset with strong generalization. In this section, we present the proposed \textbf{Temporal Dual-Depth Scoring (TDDS)} strategy, which balances the incorporation of training dynamics and the identification of well-generalized samples. In the outer level, we identify samples with their variability during training which is encouraged theoretically by the optimization space matching between coreset and original dataset (refer to Section \ref{sec: method_1}). In the inner level, the gradient in the outer level is replaced with the projected component on the accumulated direction to estimate valid contributions in every epoch (refer to Section \ref{sec: method_2}). Finally, to enhance efficiency, we conduct TDDS with a moving window (refer to Section \ref{sec: method_3}).
The proposed TDDS is summarized in \autoref{algo1}. 
\subsection{Outer Level: Enhance Coreset Generalization by Maximizing Variance}\label{sec: method_1}
To construct the coreset $\sS$ satisfying \autoref{Dataset pruning}, gradient-based methods \cite{killamsetty2021grad,mirzasoleiman2020coresets, balles2022gradient} propose to minimize the distance between full dataset and coreset gradient,
% \begin{equation}
% \begin{aligned}\label{eq: gradient matching}
% \sS^{*} = \argmin_{\sS \subset \sU}& \|\bm{G}_{t,\sU}-\bm{G}_{t,\sS}\|,\quad \mbox{where}\\
% \bm{G}_{t,\sU}=\sum_{\substack{n=1,\bm{x}_n \in \sU}}^{|\sU|}  \bm{g}_t(\bm{x}_n), \quad
% &\bm{G}_{t,\sS}=\sum_{\substack{m=1,\bm{x}_m \in \sS}}^{|\sS|}  \bm{g}_t(\bm{x}_m).
% \end{aligned}    
% \end{equation}
\textcolor{black}{
\begin{align}
\label{eq: gradient matching}
\sS^{*} = \argmin_{\sS \subset \sU}& \|\bm{G}_{t,\sU}-\tilde{\bm{G}}_{t,\sS}\|,\quad \mbox{where} \notag \\
\bm{G}_{t,\sU}=\sum_{\substack{n=1, \\ \bm{x}_n \in \sU}}^{|\sU|}  \bm{g}_t(\bm{x}_n), \quad
&\tilde{\bm{G}}_{t,\sS}=\sum_{\substack{m=1, \\\bm{x}_m \in \sS}}^{|\sS|}  \bm{g}_t(\bm{x}_m), 
\end{align}
$\tilde{\bm{G}}_{t,\sS}$ can be regarded as the gradient reconstruction in coreset space.} To solve this minimization problem, \citet{huang2023efficient} prunes samples with smaller gradient magnitudes to minimize their potential impact on optimization.

However, whenever the distance is minimized, the obtained snapshot-based coreset fails to generalize across training progress. Here are the reasons: (1) the distinctive contributions of samples are temporal statistics. Evaluating them at a specific time point causes significant bias when considering dynamic optimization; (2) samples with larger individual gradients dominate the matching process. Without considering the current optimization context, these samples introduce a substantial error in approximating the accumulated gradient.

To address the first issue, we proposed to extend \autoref{eq: gradient matching} to a continuous training duration to capture training dynamics,
% \begin{equation}
% \begin{aligned}\label{optimization matching}
% \sS^{*} &= \argmin _{\sS \subset \sU} \frac{1}{T}\sum_{t=1}^{T}\|{\bm{\mathcal{G}}}_{t, \sU}-{\bm{\mathcal{G}}}_{t, \sS}\|^2,
% \end{aligned}    
% \end{equation}
\textcolor{black}{
\begin{equation}
\begin{aligned}\label{optimization matching}
\sS^{*} &= \argmin _{\sS \subset \sU} \frac{1}{T}\sum_{t=1}^{T}\|{\bm{\mathcal{G}}}_{t, \sU}-\tilde{\bm{\mathcal{G}}}_{t, \sS}\|^2,
\end{aligned}    
\end{equation}
Here, the gradients generated by $\sU$ at epoch $t$ are defined as $\bm{\mathcal{G}}_{t, \sU}=[|\bm{g}_t(\bm{x}_n)|]_{n=1}^{N}$ and similarly $\tilde{\bm{\mathcal{G}}}_{t, \sS}$ is its reconstructed counterpart using $\sS$. Here we use magnitude instead of gradient itself to balance the training dynamic integration and complexity.
Experiments in Section \ref{sec: Ablation} also shows that magnitude-based minimization performs better than gradient-based when considering continuous training. }

Directly solving \autoref{optimization matching} is NP-hard. Thus, we turn to its equivalent, temporal gradient variance maximization,
\begin{equation}
\begin{aligned}\label{variance}
\mathbb{S}^{*} = \argmax _{\sS \subset \sU} \gR(\sS), 
\quad 
\gR(\sS) = \sum_{t=1}^{T}\|\bm{\mathcal{G}}_{t, \sS}-\overline{\bm{\mathcal{G}}}_{\sS}\|^2,
\end{aligned}    
\end{equation}
\textcolor{black}{where $\overline{\bm{\mathcal{G}}}_{ \sS}=\frac{1}{T}\sum_{t=1}^T\bm{\mathcal{G}}_{t, \sS}$, $\bm{\mathcal{G}}_{t, \sS}=[|\bm{g}_t(\bm{x}_m)|]_{m=1}^{M}$ is the mean gradient over training time.}
Detailed proof can be founded in Supplementary. \autoref{variance} measures the variability of samples and enhances the identification of well-generalized samples compared to previous average-based methods \cite{toneva2018an, pleiss2020identifying}. 
\subsection{Inner Level: Estimate Actual Contribution with Projected Gradient}\label{sec: method_2}
\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{figs/projection.pdf}
    \caption{Incorporating sample-wise gradient in the current optimization context. After projecting onto the current accumulated gradient, samples with similar gradients exhibit different behaviors.}
    \label{fig: projection}
\end{figure}
According to \autoref{variance}, sample importance can be evaluated with its gradient variance over time. For any sample $\bm{x}_n$, we have,
\begin{equation}
\begin{aligned}\label{variance_sample}
\gR(\bm{x}_n) = \sum_{t=1}^{T}\||\bm{g}_t(\bm{x}_n)|-\overline{|\bm{g}(\bm{x}_n)|}\|^2,
\end{aligned}    
\end{equation}
where $\overline{|\bm{g}(\bm{x}_n)|}=\frac{1}{T}\sum_{t=1}^T|\bm{g}_t(\bm{x}_n)|$. \autoref{variance_sample} 
treats sample-wise gradient independently, which may not precisely describe the valid contribution in the current optimization context. That is the second problem mentioned in Section \ref{sec: method_1}. As illustrated in \autoref{fig: projection}\textcolor{red}{(a)}, the gradient of sample $\bm{x}_n$ remains constant between $t$ and $t+1$. However, when incorporating it into the current optimization context, its valid contribution undergoes a significant shift. Thus, we propose to calculate the gradient variance after projecting it on the accumulated direction, that is, $|\bm{g}_t(\bm{x}_n)|$ is replaced by,
\begin{equation}\label{projection}
\begin{aligned}
|\bm{g}_t(\bm{x}_n)| &\Leftarrow
|\bm{g}_t(\bm{x}_n)\cdot\sum_{\substack{j=1,\bm{x}_j \in \sU}}^{|\sU|}  \bm{g}_t(\bm{x}_j)|.
\end{aligned}    
\end{equation}

Calculating \autoref{variance_sample} requires sample-wise gradients over a period of $T$, which is not feasible due to time and memory constraints. According to \autoref{SGD}, the accumulated gradient is equal to $\frac{1}{\eta}(\bm{\theta}_t-\bm{\theta}_{t+1})$, thus the projection in \autoref{projection} is reformed as loss difference,
\begin{equation}
\begin{aligned}\label{approximat gradient}
|\bm{g}_t(\bm{x}_n)| = &\frac{1}{\eta}|(\bm{\theta}_{t}-\bm{\theta}_{t+1})\nabla_{\bm{\theta}_{t}}\ell\left(f_{\bm{\theta}_t}(\bm{x}_n), \bm{y}_n \right)|
\\\approx&\frac{1}{\eta}|\ell\left(f_{\bm{\theta}_{t+1}}(\bm{x}_n), \bm{y}_n \right)-\ell\left(f_{\bm{\theta}_{t}}(\bm{x}_n), \bm{y}_n \right)|,
\end{aligned}    
\end{equation}
which can be deduced from the first-order Taylor expansion. 

Thus, we can evaluate the per-sample contribution to the accumulated gradient direction with its loss change. In the context of classification, $\ell$ is typically Cross Entropy (CE) loss,
\begin{equation}\label{R ce}
\begin{aligned}
\Delta\ell_t^n= \bm{y}_n^\top\cdot log\frac{f_{\bm{\theta}_{t+1}}(\bm{x}_n)}{f_{\bm{\theta}_{t}}(\bm{x}_n)},
\end{aligned}
\end{equation}
where $\Delta\ell_t^n = \ell\left(f_{\bm{\theta}_{t+1}}(\bm{x}_n), \bm{y}_n \right)-\ell\left(f_{\bm{\theta}_{t}}(\bm{x}_n), \bm{y}_n \right)$. Due to the one-hot $\bm{y}_n$, non-target probabilities are unfortunately overlooked, obliterating a significant amount of distinctive information. This reminds us of the Kullback-Leibler (KL) divergence loss, which can be achieved by simply replacing $\bm{y}_n$ with $f_{\bm{\theta}_{t+1}}(\bm{x}_n)$,
\begin{equation}\label{loss kl}
\begin{aligned}
\Delta\ell_t^n = f_{\bm{\theta}_{t+1}}(\bm{x}_n)^\top\cdot log\frac{f_{\bm{\theta}_{t+1}}(\bm{x}_n)}{f_{\bm{\theta}_{t}}(\bm{x}_n)}.
\end{aligned}
\end{equation}
Considering that $f_{\bm{\theta}_t(\bm{x}_n)}$ follows a Bernoulli distribution $\mathcal{B}(p_t)$, where $p_t$ represents the probability of the target class at epoch $t$. If $p_t$ equals $p_{t+1}$, \autoref{R ce} fails to distinguish, but \autoref{loss kl} can still differentiate the contributions of samples with $q_t$ and $q_{t+1}$. Here, $q_t$ and $q_{t+1}$ are the non-target probability distributions. This effectiveness has been proved in Section \ref{sec: Ablation}.
% , and it holds that $q_t + p_t = 1$ and $q_{t+1} + p_{t+1} = 1$
\subsection{Efficient Implementation of TDDS}\label{sec: method_3}
When computing $\gR(\bm{x}_n)$ with \autoref{variance_sample}, \autoref{approximat gradient}, and \autoref{loss kl}, storing $T$-epoch predicted outputs may lead to out-of-memory problems, especially with large datasets like ImageNet (containing \(1,281,167\) samples across \(1,000\) classes). As a solution, we suggest an efficient calculation using an exponential moving average (EMA) weighting strategy. For any training point $t\geq K$, the variance ${\gR}_t(\bm{x}_n)$\footnote{The constant coefficient $\eta$ has been omitted.} is computed over a $K$-epoch window ranging from $t-K+1$ to $t$,
\begin{equation}\label{window_variance}
\begin{aligned}
{\gR}_t(\bm{x}_n)&= \sum_{t-K+1}^{t}\||\Delta\ell_t^n|-\overline{|\Delta\ell_t^n|}\|^2,
\end{aligned}
\end{equation}
where $\overline{|\Delta\ell_t^n|}$ is the average of loss difference in a window. For $T$-epoch trajectory, $T-K+1$ windows are weighted as,
\begin{equation}\label{average R ema}
\begin{aligned}
\gR(\bm{x}_n) &=\beta {\gR}_t(\bm{x}_n)+(1-\beta)\gR(\bm{x}_n),
\end{aligned}
\end{equation}
where $\beta$ is the decay coefficient of EMA whose setting is examined in Section \ref{sec: para}. With this EMA, we only need to store predicted outputs for one window, significantly alleviating storage burden.

After sorting $\{\gR(\bm{x}_n)\}_{n=1}^N$, the top-M samples are selected to construct coreset denoted as $\{\mathbb{S}, r \} = \{\left(\bm{x}_m, \bm{y}_m\right), \gR(\bm{x}_m)\}_{m=1}^{M}$. Since, the samples with larger $\gR(\bm{x}_m)$ contribute more in the original data training. We remark that this dominance should be maintained in coreset training, i.e.,
\begin{equation}\label{subset_training}
\begin{aligned}
\bm{\theta}_{t+1}=\bm{\theta}_{t}-\eta \sum_{m=1}^M \bm{g}_t(\bm{x}_m)\gR(\bm{x}_m).
\end{aligned}
\end{equation}
This helps to transfer relative sample importance to coreset training. This effectiveness is proved in Section \ref{sec: Ablation}.
\begin{algorithm}
	\caption{Temporal Dual-Depth Scoring (TDDS)}
	\label{algo1}
 \begin{minipage}{0.99\linewidth}
	  {\bf Input:} Training dataset $\sU$; A network $f_{\bm{\theta}}$ with weight $\bm{\theta}$; Learning rate $\eta$; Epochs $T$; Iterations $I$ per epoch; Window size $K$; Decay factor $\beta$.
	\begin{algorithmic}[1]
            \FOR{$t=1$ to $T$}
            % \COMMENT{$e$ represents the current epoch}
            \FOR{$i=1$ to $I$, Sample a mini-batch $\sB_i \subset \sU$}
		\STATE Record predicted probabilities $f_{\bm{\theta}_t}(\bm{x}_n)$, $\bm{x}_n \in \sB_i$
           \STATE Calculate $\Delta\ell_t^n$ for each $\bm{x}_n \in \sB_i$
            \\ \COMMENT{Defined in \autoref{loss kl}} %\hyperref[loss difference]{Equation }\ref{loss difference} and
            \STATE Update weight $\bm{\theta}_{i+1}=\bm{\theta}_{i}-\eta \bm{G}_{t,\sB_i}$
            \ENDFOR
            \IF{$K\leq t\leq T$}
            \STATE Calculate ${\gR}_{t}(\bm{x}_n)$ in one window, $\bm{x}_n \in \sU$\\
            \COMMENT{Defined in \autoref{window_variance}}
            \STATE Update ${\gR}(\bm{x}_n)$ with EMA, $\bm{x}_n \in \sU$\\
            \COMMENT{Defined in \autoref{average R ema}}
            \ENDIF
            \ENDFOR
		\STATE Select Top-M $\{\mathbb{S}, r \}\leftarrow\{\left(\bm{x}_m, \bm{y}_m\right), {\gR}(\bm{x}_m)\}_{m=1}^{M}$
	\end{algorithmic}
 \end{minipage}
	\hspace*{0.02in} {\bf Output:} Selected subset $\mathbb{S}=\left\{\left(\bm{x}_m, \bm{y}_m\right)\right\}_{m=1}^M$; associated sample-wise importance $r=\{{\gR}(\bm{x}_m)\}_{m=1}^{M}$
\end{algorithm}
